The shocklet transform: A decomposition method for the identification of local, mechanism-driven dynamics in sociotechnical time series

We introduce a qualitative, shape-based, timescale-independent time-domain transform used to extract local dynamics from sociotechnical time series---termed the Discrete Shocklet Transform (DST)---and an associated similarity search routine, the Shocklet Transform And Ranking (STAR) algorithm, that indicates time windows during which panels of time series display qualitatively-similar anomalous behavior. After distinguishing our algorithms from other methods used in anomaly detection and time series similarity search, such as the matrix profile, seasonal-hybrid ESD, and discrete wavelet transform-based procedures, we demonstrate the DST's ability to identify mechanism-driven dynamics at a wide range of timescales and its relative insensitivity to functional parameterization. As an application, we analyze a sociotechnical data source (usage frequencies for a subset of words on Twitter) and highlight our algorithms' utility by using them to extract both a typology of mechanistic local dynamics and a data-driven narrative of socially-important events as perceived by English-language Twitter.

==> sections/realtime.tex <==
\section{Real-time classification} \label{sec:realtime}

Though the DCuT is able to extract interesting dynamical behavior from sociotechnical time series, 
if used in a real- or near-real-time classification context it suffers from the major flaw of noncausality, 
since it can be written as a function of the form 
$y(t) = f(x_{t + W/2},...,x_{t - W/2})$,
where 
$$
y(t) = \begin{cases} 
1 & \quad \text{in a cusp window} \\ 
\end{cases}
.
$$
We require an estimated model $\hat{f}(x_t, x_{t-1},...,x_{t - W})$
that minimizes a loss function $L(y(t), \hat{f}(x_t, x_{t-1},...,x_{t - W}))$.
This is accomplished by training a supervised machine learning algorithm to predict
$\mathrm{C}_{\mathcal{K}}(t)$ from $x_t,...,x_{t - W}$ and applying an approximate weighting scheme. 
\begin{figure*}[!h]
	\centering
	\includegraphics[width=\textwidth]{figures/mlp_realtime_panel_example.pdf}
	\caption{
		Comparison of the true cusplet indicator function and its associated cusp windows with the learned 
		real-time cusplet indicator function and its associated windows.
		The top row of figures displays the indicator functions, 
		while the bottom row of figures shows the original rank time series along with the cusp windows 
		from the two algorithms.
		From left to right, the columns correspond to the words "trump", "gaza", and "hurricane".
		The color blue denotes the real cusplet indicator, while the color red denotes the learned real-time 
		indicator.
		}
	\label{fig:mlp_realtime_panel_example}
\end{figure*}
The resulting causal cusp indicator is able to reproduce the results of the DCuT while not suffering from edge
effects in real-time use.



The model used in the construction of the real-time cusp indicator is a deep neural network.
Deep neural networks have the universal (continuous) function approximation property and thus are useful for 
complex, non-linearly-separable problems
\cite{hornik1991approximation}.
The network used here was composed of an input layer with dimensionality equal to $W_{\max} = 748$,
two hidden layers of 200 and 100 nodes respectively, and a single output neuron.
Rectified linear units are used as activation functions, except for the output node, which uses a linear output.
The network was trained until the validation score did not improve by more than 
$\Delta R^2 = +1\times 10^{-4}$ for 10 consecutive epochs, 
for a total of 101 epochs, using stochastic gradient descent with Nestorov's momentum adaptation 
\cite{nesterov1983method}.
\begin{figure*}
\centering
	\includegraphics[width=\textwidth]{figures/ranked_cusp_weighted_realtime.pdf}
	\caption{}
	\label{fig:ranked-cusp-weighted-realtime}
\end{figure*}
